Accelerating Fully Connected Neural Network on Optical Network-on-Chip (ONoC)

Fully Connected Neural Network (FCNN) is a class of Artificial Neural Networks widely used in computer science and engineering, whereas the training process can take a long time with large datasets in existing many-core systems. Optical Network-on-Chip (ONoC), an emerging chip-scale optical interconnection technology, has great potential to accelerate the training of FCNN with low transmission delay, low power consumption, and high throughput. However, existing methods based on Electrical Network-on-Chip (ENoC) cannot fit in ONoC because of the unique properties of ONoC. In this paper, we propose a fine-grained parallel computing model for accelerating FCNN training on ONoC and derive the optimal number of cores for each execution stage with the objective of minimizing the total amount of time to complete one epoch of FCNN training. To allocate the optimal number of cores for each execution stage, we present three mapping strategies and compare their advantages and disadvantages in terms of hotspot level, memory requirement, and state transitions. Simulation results show that the average prediction error for the optimal number of cores in NN benchmarks is within 2.3%. We further carry out extensive simulations which demonstrate that FCNN training time can be reduced by 22.28% and 4.91% on average using our proposed scheme, compared with traditional parallel computing methods that either allocate a fixed number of cores or allocate as many cores as possible, respectively. Compared with ENoC, simulation results show that under batch sizes of 64 and 128, on average ONoC can achieve 21.02% and 12.95% on reducing training time with 47.85% and 39.27% on saving energy, respectively.

==> modext.tex <==
\vspace{-2mm}

\section{Model Extensions} \label{sec:extension}
In this section, we illustrate how our proposed model and method can be extended to other topology such as torus and other type of neural network such as CNN, which shows the scalability of our model.   
%Our proposed model and methods are scalable and extendable. We illustrate the basic ideas for model extension to other topology with larger batch-size and model extension to other ANNs  
\vspace{-2mm}
\subsection{Extension to Torus Topology for Better Scalability}
When the number of cores increases in an ONoC, mesh or torus is commonly used to achieve better scalability \cite{dong2010multiple}. As shown in Fig.~\ref{fig:extension}, a 2D torus is a 2D mesh by 
adding wrap-around edges to directly connect the end nodes in each row and column. Hence, all nodes in each row forms a ring, and we call it a horizontal ring. All nodes in each column also forms a ring, and we call it a vertical ring.  In the following, we explain how our model and method can be extended to torus topology. %when the batch size is no smaller than the number of rows in an ONoC with a torus topology. 
\begin{figure}[!ht]
	\vspace{-3mm}
	\centering
	\includegraphics[scale=0.65]{extension11.pdf}
	{
		\vspace{-1mm}
		\caption{Model extension to torus topology}
		\label{fig:extension}
	}
\end{figure}
%
Firstly, the training samples in one epoch are evenly assigned to the horizontal rings as different lines of samples, which can be processed in parallel according to our proposed FCNN acceleration method. During the FP process, all FCNN samples in the horizontal rings perform computation and communication based on our proposed method. During the BP process, each neuron needs to calculate the gradients propagated back to the previous layer to update the weights. 
%When processing sample number of per horizontal ring is larger than 1, the weights are updated per epoch instead of per sample.
Since all FCNN samples in horizontal rings are mapped in the same way based on our proposed method, 
%the corresponding neurons must be mapped to the same core in all the horizontal rings, that is, the neurons mapped to each core in the same vertical ring is the same. Therefore, 
each core in a vertical ring stores parameters of the same neurons for one batch, which requires to synchronize the updated parameters for each neuron among all FCNN samples mapped to the horizontal rings. Hence, the synchronization of updating parameters can be achieved using optical communications in each vertical ring. Fig.~\ref{fig:extension} gives an example based on RRM strategy, where the cores with the same color are allocated for the same period.

%In the Fig.~\ref{fig:extension}, cores in light blue and blue run in the first period and second period separately and cores in green color run at the third period in the FP process.

%Our method on core allocation, neuron mapping and wavelength allocation  in each horizontal ring. 
%
%\noindent When the number of cores is increasing, the ring, mesh and torus are very common topology to use for ONoC \cite{dong2010multiple}. Our proposed model is based on the ring topology, however, it can also be extended to mesh, torus or other topology with the batch-size of input is larger or equal to 2. Assume an ANN is training in a 30 core torus ONoC by using our proposed model in Round-robin mapping and the batch-size is 5. As illustrated in Fig.~\ref{fig:extension}, during the FP process, each row of the torus is executing one training example and applied our accelerating scheme with 2 cores in gray color assigned to period 1, 3 cores in blue color assigned to period 2 and 1 core in green color assigned to period 3. While in the BP process, each column of the cores in each period need to do all to all multi-cast so that the updated parameters of each the layer are synchronized. Since each row and column of ONoC have no shared ONoC links when they execute in parallel for one training example based on our proposed methods, they can use the same wavelength in its row and column. 


%\noindent In this section we illustrate the scenario when the batchsize of input is larger or equal to 2. When set with batchsize, ONoC is divided into several parts according to the batchsize number and each part of ONoC execute the parallel computation simultaneously using the above proposed method of batchsize = 1. 

%The $Time_1$ is equal to the maximum FP time of subgroup plus one computation of the average parameters and communication between the two subgroups. But there is a little difference that after the two groups finish its computation, two groups will both store all neuron's parameters in the shared memory, then two group's parameters is conduct average calculation and update them to the shared memory. $f_{1}(\sigma_{ln}, C)$ equals to the time of cores to do the average calculation of all the parameters of neurons and $E_{ln}$ is the delay of read all the outcome of neurons and after average calculation write these outcome of neurons to the shared memory.Since we have divided the Ring-based ONoC into a few subgroups to execute parallel computation. Each of the subgroup actually is doing parallel computation using the method we mentioned in the Section V. As a result, each subgroup actually can reuse the wavelength in there communication process because their communication is separative in the FP process. When ONoC is divided into two subgroups, each subgroup read a input and the cores in the subgroup do parallel computation by using our proposed parallel method. After they finish computation, the two neural networks parameters need to average and store in the shared memory for the back propagation.

%We use the same sample ANN Fig.~\ref{fig:neural-new} trained in a 18 cores ONoC chip to do the demonstration. We assume the input batchsize is 2 and the optimal assigned core list is the [3, 4, 5, 3]. Then ONoC will be divided into two groups and the CRPM algorithm is used in each subgroup. After the cores are mapped with input and ANN, each subgroup will parallel training separately. In here we show the communication process of two subgroups in the period 1, as can be seen in Fig.~\ref{fig:ring6}. 

%During the back propagation, the gradients of the current layer is got and the weights and bias will be updated and write through to the shared memory across periods asynchronously. When finishing all the training of two subgroups, all the updated of parameters of the model are stored distributively in the cores of two groups and the shared memory. Then, there will be one more step for the extension model to get the updated parameters of this batch size, which is to average the weights and biases got from two subgroups. 

%In computation period 3 the assigned core number is 4 and the computation period 4 the assigned core number is 2, the computation cores list of subgroup 1 in period 3 would be [core 4, core 5, core 6, core 7] and the core list in period 4 is [core 6, core 7] according to the CRPA-E algorithm. In subgroup 2, the situation is similar except the index is different. 
%Let us cite a real example to describe it. let us say there are 100 pictures(whole dataset), and each iteration the neural network is fed two pictures to train. Actually, the two pictures could be parallel training because their computation is separated. After they finish computation and get their loss, their loss and each neuron's parameters will be average in this iteration. Then backward propagation will be executed.


\subsection{Model Extension to CNN}
Since FCNN, CNN and other neural networks all have FP and BP processes with basic multilayer structure, our approach can be extended to other neural networks, provided the neural network is properly partitioned into sub-networks with balanced computation and communication loads. Then our model can be used to map the neurons to cores for parallel neural network training, and the communications can be realized using optical transmissions on ONoCs.  

%Assuming that the network of CNN or RNN is optimally partitioned, with our approach we can derive the optimal assignment of cores for each period using our mapping algorithm. 


%Since the MLP, CNN, RNN and other neural networks all have FP and BP processes with basic multilayer structure, our approach can be extended to other neural networks, provided the neural network is properly partitioned into sub-networks with balanced computation and communication loads. Then the workloads are mapped to cores to perform ANN training in parallel, and the communications can be achieved by using optical transmissions on ONoCs. Assuming that the network of CNN or RNN is optimally partitioned, with our approach we can derive the optimal assignment of cores for each period using our mapping algorithm. 
%However, the partitioning of the network, an NP hard problem, is outside the scope of this paper.
As we know, fully connected layer can be used in CNN that takes the result of convolution/pooling process and reaches a classification decision. When extending our model to CNN, we only need pay attention to the convolution (weights sharing) and pooling operations in CNN. In convolution layer, the sample input is executed with convolution operation by using the filter to get the feature map. In pooling layer, feature map obtained from convolution layer is executed with pooling operation, with the result of reducing the size of feature map to obtain the main feature. 
The convolution computation is most time-consuming in the CNN training, which can be partitioned and distributed to different cores to conduct parallel computation. For instance, 3D input of CNN can be divided by either one dimension sequential partitioning or cross-dimension partitioning method, and etc., and the corresponding filters are mapped to cores to conduct parallel computation and get the partial sums. After that, instead of sending partial sums to the main memory, cores worked in the last period send partial sums to cores that will work in next period to conduct parallel computation of the next layer. These computations and communications of different cores occur alternately during different training periods. 
Therefore, the communication pattern during these periods in CNN training has some similar characteristics with the communication pattern of FCNN, thus our model can be further extended to work for CNN by simplifying and modifying the communication patterns and the corresponding mapping method.
%gather partial sums from the part of cores worked in last layer and then proceed the computation of next layer and so on and so forth.
%The main difference between MLP and RNN is that RNN uses shared weights and takes into account what happens before by adding a looping constraint on the hidden layer. The neurons in all hidden state use the same weights and the output of the neuron in the current hidden state will be the input of the next hidden state. This requires communications among neurons in the same layer. Our model can be easily extended to work for RNN by adding an extra component to model the intra-layer communication/computation pattern within each period for RNN training.

%, whereas the solution to compute the optimal number of cores per period and the mapping strategies remain unchanged. 



%We build up an ANN accelerating model which considers a trade-off between computation and communication based on MLP workload by dividing MLP into periods according to the MLP layers. Since the MLP, CNN, RNN and other neural networks all have FP and BP computation process and basic structure of multilayer, we can extend our approach to other neural networks, provided the network is properly partitioned into subnetworks with balanced computation and communication loads. Then the workloads are mapped to cores to perform ANN training in parallel. Assuming that the network of CNN or RNN is optimally partitioned, with our approach we can get the optimal assignment of cores in each period using our mapping algorithm. However, the partitioning of the network, an NP hard problem, is outside the scope of this paper.
%Specifically, the main difference between MLP and CNN are the convolution operation and the pooling operation. The former operation uses the shared weights to get the feature map and the latter one can reduce the size of parameters and computation, so that the condensed feature map can be obtained.  Actually, the CNN computations can flatten into MLP-like CNN~\cite{chen2019noc}, thus the convolution and pooling computation of CNN can be converted to the MLP computation. So we can just modify our proposed model a little bit and get a compatible CNN accelerating model on ONoC. As for RNN, the each neuron in a given layer is connected with a directed connection to every other node in the next successive layer and rely on the consecutive data, such as audio, video, text, etc. 




















==> motiv.tex <==
\vspace{-2mm}
\section{Motivating Examples}\label{sec:motivation}

In this section, we first explain how a MLP can be trained in an ONoC, and then present the motivations of our solution that leverages ONoC to accelerate MLP training. 

We use the example given in Fig. \ref {fig:neural-new} (a) to explain the process of MLP training in an ONoC. To speed up training using parallel computation, the neurons in the MLP are firstly mapped to distributed SRAM of cores on the ONoC, where multiple neurons can be mapped onto the same core. As illustrated in Fig. \ref {fig:neural-new} (a), one epoch of training is divided into multiple periods based on layers, and these periods are executed sequentially. 
In \textit{Period 0}, data and instructions of MLP in hard disk are mapped and loaded by main memory and then by SRAM of ONoC cores.
Then, in each following period, the cores mapped with neurons in the corresponding layer perform computations concurrently and then pass the outputs to the cores mapped with neurons in the next layer through inter-core communications. Thus, great latency of frequent access shared memory can be saved.

\begin{figure}[!ht]
	\vspace{-1mm}
	\centering
	\includegraphics[scale=0.35]{neural-new1.pdf}
	{
		\vspace{-2mm}
		\caption{Illustration of neural network training on ONoC; (a) Periods of neural network; (b) Using 2 cores in Period 1 by scheme 1, the two cores can implement concurrent communications within one time slot; (c) Using 4 cores in Period 1 by scheme 2, two cores conduct concurrent communication in first time slot, and (d) other two cores conduct concurrent communication in first time slot due to wavelength limitation.}
		\label{fig:neural-new}
	}
\end{figure}

%multi-core \noindent When given an ANN and an ONoC, such as Fig.\ref {fig:neural-new}, mapping ANN to ONoC is the first step of ANN training on ONoC. We divide the ANN into 8 periods according layers as can be seen in Fig.\ref {fig:neural-new} (a), where forward propagation of ANN occupies first four periods and the back-propagation occupies the next four periods. In the mapping process, the neurons in the different layer will map to the different parts of ONoC cores. Afterwards, the ANN training in ONoC will be proceeded by parallel computation and communication between cores alternately across the periods. 
With such a mapping of MLP training on ONoC, we illustrate our key motivations using the following examples: 

%use the following examples to show the key motivations of our approach:  Example I shows that ONoC has great potential 
%to accelerate ANN training by taking the advantages of optical transmission for data exchange between cores in adjacent periods. 
%Example II illustrates that there is a tradeoff between computation and communication for ANN training on ONoC, which allows the use of optimization techniques to further 
%reduce the amount of time required to train a neural network. 
%The main difference between the shared memory architecture and the distributed memory is the data acquisition channel 
\vspace{-1mm}
\noindent\textbf{Example I}: This example is to illustrate \textit{MLP training can be accelerated by exploiting optical transmission for data exchange between cores in adjacent periods}. When a MLP is trained in a traditional multi-core system with shared memory, the outputs of each neuron, weights, biases and gradients need to be written to the shared memory. When the neurons in two adjacent periods are not mapped to the same core, the data needed for the computation in the next period must be read from the shared memory to the corresponding cores. If the cores are reading the same parameters in the shared memory, more delay will occur in the shared memory due to bank or port conflict. 
These frequent read and write operations in shared memory will cause great delay, thereby slowing down the MLP training process. 
For example, it takes around 180 cycles to access shared memory in three level cache intel i7 CPU~\cite{levinthal2009performance}. Accessing the GPU shared memory and global memory takes about 30 cycles and 375 cycles, respectively in the NVIDIA Volta gpu architecture~\cite{jia2018dissecting}. 
However, the off-chip memory access for MLP training can be alleviated by 88.1\% using on-chip inter-core communication~\cite{chen2019noc}.
The average latency of inter-core communication ranges from 19 to 91 cycles in ENoC~\cite{catania2006methodology} and 3 to 7 cycles in ONoC~\cite{morris20123d}, which are much faster than shared memory access. Obviously, in comparison with ENoC,  ONoC has much more potential to reduce the amount of time required for data communication during MLP training.
Moreover, by leveraging the WDM technology, multiple cores connected with waveguide can transmit and receive data concurrently as long as they use different wavelengths. 
This can further reduce the amount of time for data communication between neurons in adjacent layers. Our study aims to explore this potential of ONoC for parallel MLP training, then extend this work to other ANNs.
%Figamount of time required for data exchange between layers can be significantly reduced. 
%
%communication delay for . 
%From the above figure comparison, cache miss of the core in traditional multi-core shared memory system will lead to read/write operation in the global/shared memory, which has tremendous latency. That is because in traditional multi-cores shared memory architecture  platform will have potential high delay due to the cache coherence and cache miss when performing parallel computation. However, those issues can greatly be avoided in the distributed memory architecture by using communication between cores. %when the first period cores finish the mapping  
%When conducting parallel ANN training in NoC, firstly, parts of ANN are mapped to the NoC cores  properly and then part of cores will execute parallel computation and communicate with other part of cores across ANN training periods without any shared memory access during the ANN training. Therefore, the delay of parallel training of ANN can be greatly reduced if properly using the NoC communication of cores. Obviously, ONoC have great advantages over ENoCs and have much more potentials to reduce the data exchange time between layers during the ANN training. Let us assume there are 100 times message passing among cores during one epoch training of ANN in ONoC. ANN training in traditional shared memory architecture is executed 100 times write and read operation in the shared memory, which is about 100 cycles for each operation. However, optical transmission time between cores is about 3~8 cycles (differ in different architecture). As a result, using ONoC transmission instead of using memory accessing in the training of ANN can save 9700 cycles (best case) in this one epoch training of ANN.

\vspace{0 mm}
\noindent\textbf{Example II}: This example is to illustrate \textit{there is a trade-off between computation and communication for MLP training on ONoC , which allows the use of optimization techniques to further reduce the amount of time required to train a neural network}. Suppose that the MLP given in Fig. \ref {fig:neural-new} (a) is trained on an ONoC with four cores connected into a ring topology. We assume that the number of available wavelengths is 2. 
Taking the execution of \textit{Period 1} as example, let us consider the following two mapping schemes between neurons and cores: (1) the four neurons are mapped to \textit{Core 1} and \textit{Core 2} with each having two neurons, as illustrated in Fig. \ref {fig:neural-new} (b) and (2) each neuron is mapped to one core, as illustrated in Fig. \ref {fig:neural-new} (c) and (d).  Since only 2 wavelengths are available, \textit{Core 1} and \textit{Core 2} can share their data with other cores in parallel using 2 different wavelengths in Scheme 1. However, in Scheme 2 TDM has to be used since only two cores can send in parallel at one time, which will cost two time slots. In the first time slot,  \textit{Core 1} and \textit{Core 2} can send their data to other cores in parallel using 2 wavelengths and \textit{Core 3} and \textit{Core 4} have to exchange their data in the second time slot, as illustrated in Fig. \ref {fig:neural-new} (c) and Fig. \ref {fig:neural-new} (d), respectively. Hence, Scheme 1 uses more time on computation with less time on communication than Scheme 2.  
%We have divided the ANN into different parts and they will be mapped to ONoC cores. Then the mapping cores in the ONoC will be proceeded parallel computation to finish the part of ANN computation then transmit the computation outcome to the cores that mapped next part of ANN, and so forth to finish the ANN training. One period instance of parallel computation and communication of ANN training can be seen in the Fig.\ref {fig:neural-new} (b). Two cores were assigned to compute layer 1 in first period and the four cores were assigned to compute the layer 2, after the two cores finish period 1 computation, core 1 and core 2 send their computation outcomes to the rest of cores. In the communication of the ONoC, since the wavelength number is limited, TDM will be used if sender number is larger than wavelength number with more communication time slot.
It can be seen that there is a trade-off between computation and communication in the mapping between neurons and cores, in order to minimize the total training time. 
Using more cores will reduce the computation time, but may incur more time on communication. \textit{The challenging problem is: to train a given MLP on an ONoC with a limited number of available wavelengths, how to map the neurons to cores to minimize the total amount of time for MLP training by exploring this tradeoff.} Traditional methods such as using a fixed number of cores all the time~\cite{zou2019learn} or using as many cores as possible to maximize parallel computation~\cite{pethick2003parallelization}, did not consider this tradeoff to optimize MLP training. Therefore, we propose a MLP acceleration model in ONoC that explores the trade-off between computation and communication to calculate the optimal number of cores for each period to minimize the MLP training time. 


